DeepLSH: Deep Locality-Sensitive Hash Learning for Fast and Efficient Near-Duplicate Crash Report Detection

Automatic crash bucketing is a crucial phase in the software development process for efficiently triaging bug reports. It generally consists in grouping similar reports through clustering techniques. However, with real-time streaming bug collection, systems are needed to quickly answer the question: What are the most similar bugs to a new one?, that is, efficiently find near-duplicates. It is thus natural to consider nearest neighbors search to tackle this problem and especially the well-known locality-sensitive hashing (LSH) to deal with large datasets due to its sublinear performance and theoretical guarantees on the similarity search accuracy. Surprisingly, LSH has not been considered in the crash bucketing literature. It is indeed not trivial to derive hash functions that satisfy the so-called locality-sensitive property for the most advanced crash bucketing metrics. Consequently, we study in this paper how to leverage LSH for this task. To be able to consider the most relevant metrics used in the literature, we introduce DeepLSH, a Siamese DNN architecture with an original loss function, that perfectly approximates the locality-sensitivity property even for Jaccard and Cosine metrics for which exact LSH solutions exist. We support this claim with a series of experiments on an original dataset, which we make available.

==> tex/introduction-yre.tex <==

\section{Introduction}\label{sec:introduction}

\begin{figure}
\centering
    \begin{lstlisting} 
        id: 16377610978254995717215-XXXXXXX-XX
        sessionId: 2D7E2416131887D473F6CFD7B35769C
        version: 13.7
        server: XXXXXXX-XX
        @timestamp: 2022-07-26 11:13:40.657
        typeError: ERROR
        functionality: com.myCompany.modules.atelier.poste.PostProdVC
        message: class com.myCompany.exceptions.MyException : No CAB matches reading: 'Invalid' 
        detail: at com.myCompany.opeOF.LancFromCABAdapter.doCreation(LancFromCABAdapter.java:449)
                at com.myCompany.tools.cab.CABWrapper$1.readDone(CABWrapper.java:191) |\Suppressnumber|
                ..... |\Reactivatenumber{29}|
                at com.myCompany.SuperviseurApp.main(SuperviseurApp.java:94)
    \end{lstlisting}
    \caption{\small Example of a crash report.}\label{fig:crashexample}
\end{figure}


%%%%%%%% quelques notes pour mehdi  pour la motivation pratico pratique
%% décrire comment on fait chez infololo : real time collection (c'est vrai !) 
%% avec enormément de bug dont certains peuvent etre très grave d'autre de la pure
%% esthétique /ergonomiue (bloquant pénible invisible mais important...)
%% bcp de versions du meme soft dans la nature et donc de stacks traces différentes
%% pour un meme pb. 
%% on souhaite avoir ranking dynamique en fonction du nombre d'occurences 
%% la premiere étape est d'avoir une similairyt super efficace car on recoit
%% x millions de stacks par jour (?).
%% plutot facile d'étudier les stacks  bloquantes car elles sont rares
%%% par contre très difficile de faire le tru dans le reste. 
%% surtout on veut rattacher une nouvelle occurence au traitement en cours ou
%% a un bug caractérisé dans notre system de maintenance. ca fournit 
%% au n2 / dev des stats précises sur l'impact d'un bug sur le parc 
% et aidrera améliorer le ranking (car d'autres métriques sont a prendre en compte, 
%% c'est du multi critère.
%% on a aussi le cas ou le client vient avec un priobleme et demande une résolution rapide, il faut etre capable de rapidement trouver les autres appels qui traite / ont traité le meme probleme. pire encore 2 personnes d'un meme client peuvent faire le meme appel en // sans le savoir, il est indispensable de ne pas traiter l'appel 2 x en //. 

%Collecting runtime errors and attempting to correct either the source code or the configuration of a software after its release is nowadays a standard process of software engineering. 



To facilitate debugging for developers, several systems such as Windows Error Reporting~\cite{DBLP:conf/sosp/GlerumKGAONGLH09} and Mozilla Crash Reporter~\cite{website:mozillaCR} have been deployed to automatically collect and triage crash reports. These reports usually contain several pieces of information relevant to the bug, mainly the stack trace, giving the precise location of the problematic code line and the function call stack, as illustrated in Figure~\ref{fig:crashexample} with a complete example of a crash report. It is noteworthy that one specific bug may produce slightly different stack traces called near-duplicates~\cite{DBLP:conf/icse/DangWZZN12}. Therefore, it is highly valuable to group similar crashes into buckets to accelerate the crash investigation process~\cite{DBLP:conf/icsm/DhaliwalKZ11}. Crash reporting systems use a range of heuristics and manually developed rules to organize crash reports into categories, ideally with each category referring to the same bug~\cite{DBLP:conf/sosp/GlerumKGAONGLH09}. However, in many scenarios, it may assign crash reports caused by the same bug to multiple buckets~\cite{DBLP:conf/sosp/GlerumKGAONGLH09}. Furthermore, implemented rules are supposed to be consistent, with good accuracy and coverage. This is not trivial as new features are constantly being introduced in software systems~\cite{DBLP:journals/corr/abs-2109-14326}. Thus, plenty of alternative methods have addressed the stack trace-based report deduplication problem by designing custom and accurate similarity measures between stack traces. Existing approaches rely mostly on string or graph matching (e.g., edit distance, prefix match and LCSS)~\cite{DBLP:conf/icsm/DhaliwalKZ11,DBLP:conf/dsn/KimZN11, DBLP:conf/icac/BrodieMLMMWCS05} and information retrieval (e.g., TF-IDF and N-grams)~\cite{DBLP:conf/csmr/LerchM13,DBLP:conf/qrs/SaborHL17}. Some other specific metrics consider the particular characteristics of stack traces (e.g., the distance to the top frame or the alignment offset between two matched frames)~\cite{DBLP:conf/sigsoft/VasilievKCKLP20, DBLP:conf/icse/DangWZZN12, DBLP:conf/seke/MorooAH17}. 

%The main challenge that we tackle is to efficiently locate nearly duplicate stack traces for a new crash report, given a large historical dataset of stack traces and for any user-defined similarity measure. More specifically, we attempt to find the most likely stack traces to be clustered in the same bucket w.r.t. any given similarity measure. This is an instance of the nearest neighbors search problem~\cite{DBLP:journals/corr/WangSSJ14}. Providing exact results is often computationally infeasible when the studied dataset is very large or the similarity measure computation is costly. 

%Significant research efforts have been directed towards the search for approximate nearest neighbors (ANN) that has proven to be enough and practical in many domains. Hashing is among the most popular techniques for ANN due to its computational and storage efficiency~\cite{DBLP:journals/corr/abs-2003-03369, DBLP:journals/corr/WangSSJ14}. It consists in projecting the data items from the original features of high-dimensionality into a low-dimensional representation, or equivalently a short code (i.e., hash code). The application of hashing for ANN includes indexing the data using hash tables constructed by storing items that share the same hash code into a hash bucket. This approach satisfies the locality-sensitive property, that is, similar items are expected to have a higher probability to be mapped into the same hash code (i.e. belonging to the same hash bucket) than dissimilar items with guarantees \cite{DBLP:journals/corr/WangSSJ14}. LSH is known for its computational and storage superiority, as well as its sub-linear search performance and theoretical guarantees on ANN search accuracy~\cite{DBLP:conf/stoc/IndykM98}. The research work in this direction focuses on the generation of a family of random hash functions for a given similarity measure that meets the locality-sensitive property. We recognize many LSH families for different conventional similarity measures or distances, including $l_p$ distance~\cite{DBLP:conf/compgeom/DatarIIM04}, angular distance~\cite{DBLP:conf/stoc/Charikar02}, and Jaccard coefficient~\cite{DBLP:journals/cn/BroderGMZ97}, etc. However, no systematic procedure have been designed to derive an LSH family of hash functions for any given similarity measure. More specifically, applying LSH on custom similarity measures to address the challenging problem of crash deduplication remains an unexplored area.

\modif{With the aim of efficiently locating nearly duplicate stack traces, given a large historical dataset of crash reports and an accurate stack trace-based similarity measure, a challenging problem of scalability has been encountered. Applying modern stack trace similarity measures in production environment scenarios, where we expect thousands of errors/exceptions to be raised daily, made us realize that these complex similarity measures do not scale. For instance, with Brodie similarity metric~\cite{DBLP:conf/icac/BrodieMLMMWCS05}, attempting to find the most similar crash reports for only $1,000$ new crashes out of $100,000$ historical crashes, the process required more than 10 hours to conduct a simple linear scan. A conclusion we have reached in this specific context, is that providing exact results is computationally infeasible when the studied dataset is very large or the similarity measure computation is costly. Consequently, our efforts have shifted towards the research area of approximate nearest neighbors search (ANN) that has proven practical and sufficient in many domains.} 

Hashing is among the most popular techniques for ANN due to its computational and storage efficiency~\cite{DBLP:journals/corr/abs-2003-03369,DBLP:journals/corr/WangSSJ14}. It consists in projecting the data items from the original features of high-dimensionality into a low-dimensional representation, or equivalently a short code (i.e., hash code), \modif{such that the similarity between the resulting hash codes remains an effective approximation/estimation of the real similarity in the original space.} The application of hashing for ANN includes indexing the data using hash tables constructed by storing items that share the same hash code into a hash bucket. This approach satisfies the \textit{locality-sensitive property}, that is, similar items are expected to have a higher probability to be mapped into the same hash code (i.e. belonging to the same hash bucket) than dissimilar items with guarantees \cite{DBLP:journals/corr/WangSSJ14}. LSH is known for its computational and storage superiority, as well as its sub-linear search performance and theoretical guarantees on ANN search accuracy~\cite{DBLP:conf/stoc/IndykM98}.  \modif{The challenge in using LSH for crash deduplication lies in generating a family of random hash functions for a given similarity measure that meets the locality-sensitive property. Although a diverse set of LSH family functions have already been proposed, each for estimating one and only one conventional similarity/distance measure, e.g., Min-Hash function for Jaccard coefficient~\cite{DBLP:journals/cn/BroderGMZ97} and Sign-Random-Projection (Sim-Hash) function for angular distance~\cite{DBLP:conf/stoc/Charikar02}, etc., it remains ambiguous and theoretically difficult to generalize this procedure to other similarity measures. Specifically, there is no systematic procedure for deriving a family of LSH hash functions for a given similarity measure. Therefore, applying LSH to custom similarity measures to solve the challenging problem of efficient and scalable crash deduplication remains an unexplored area. To overcome the aforementioned problems, we propose to learn these hash functions in a supervised manner to mimic any given similarity measure, while incorporating the locality-sensitive hashing component into the model learning process. 

Learn to hash~\cite{DBLP:conf/cvpr/LiongLWMZ15,DBLP:conf/cvpr/Liu0SC16,DBLP:conf/nips/LiSHT17,DBLP:conf/eccv/DoDC16,DBLP:conf/cvpr/LaiPLY15,DBLP:conf/accv/WangSK16} on the other hand, has been widely attracting a large research community, primarily in computer vision. These techniques are highly effective in reducing the dimentionality of the input data representations while preserving their similarities. However, they do not meet our main objective which consists in an end-to-end procedure to retrieve near-duplicate data objects with guarantees. These techniques do not reveal a systematic way to construct hash tables from the resulting hash codes, and neither do they control the trade-off between recall and precision using key hyperparameters as does LSH. To achieve our goal which consists in fast, efficient and scalable near-duplicate crash report detection given any similarity measure, we take benefit from both worlds, i.e., LSH and Learn to Hash.} We propose an approach that learns to approximate a family of diverse LSH functions for any user-defined similarity measure, using a deep Siamese neural network by incorporating the locality-sensitive property into the loss function. These hash functions are then used to quickly and efficiently find similar items that share the same subset of a hash code. To this end, we address two main challenges: (1) how to formalize the locality-sensitive property in the objective loss function? (2) how to deal with the binarization constraint in the hash codes during the learning phase? \modif{Note that our approach does not propose a new similarity measure and does not question the effectiveness or evaluate the proposed similarity measures, but rather improve the use of LSH to enhance the ANN search with respect to these similarity measures.} To the best of our knowledge, there has been no prior work that incorporates Hashing in general and LSH in particular for the crash deduplication problem. The most similar baseline has been outlined in \cite{DBLP:journals/tip/HuFXSCM18} since it is the only existing approach to combine Deep Learning and LSH. However, the adopted methodology is significantly different to ours, where the authors proposed a deep constrained hash coding network for near-duplicate image detection. However, unlike our proposal, their approach initially entails deep hashing to learn the similarity, and then performs separately in a second phase LSH on the resulting vectors which compromise the search accuracy as shown in our experimental study, since the LSH has not been incorporated into the model to mimic the similarity (more details are provided in the RW Sec~\ref{sec:relatedwork}). We summarize our contributions as follows:

\begin{itemize}
    \setlength\itemsep{0.2em}
    \item \modif{To the best of our knowledge, we are the first to employ hashing in general and LSH technique in particular to address the problem of crash deduplication, given a large dataset of stack traces and for any given user-defined similarity measure.}
    
    \item Aiming to overcome the challenging problem of deriving LSH functions for stack trace-based similarity measures, we propose a generic approach dubbed \texttt{DeepLSH} that learns and provides a family of binary hash functions that almost perfectly approximate the \textit{locality-sensitive property} to retrieve efficiently and rapidly near-duplicate stack traces.% with approximate guarantees.
    
    \item \modif{Technically, we design a deep Siamese neural network architecture to perform end-to-end hashing with an original objective loss function based on the locality-sensitive property preserving with appropriate regularizations to cope with the binarization problem of optimizing non-smooth loss functions with binary constraints.} 
    
    \item We demonstrate through our experimental study in Sec~\ref{sec:xp} on a large real-world stack trace dataset that we provide from our ERP software under $12$ different similarity metrics the effectiveness and scalability of \texttt{DeepLSH} to yield near-duplicate crash reports compared to standard LSH techniques, particularly, MinHash and SimHash, and the most relevant identified deep hashing baseline~\cite{DBLP:journals/tip/HuFXSCM18}.     
\end{itemize}

%We summarize our contributions in this paper as follows: (1) We train a  Siamese neural network for stack traces to perform end-to-end hashing task with a custom loss function based on locality-sensitive property preserving w.r.t. any given similarity measure. (2) We extract directly from the neural network a family of binary hash codes to be used to access hash tables with a sub-linear time complexity. (3) We conduct our experimental study on a large dataset of stack traces to evaluate the model effectiveness in providing appropriate hash codes for efficient ANN search under $10$ different similarity measures proposed in the context of crash deduplication problem.

==> tex/replication.tex <==
\section{Data and Code Availability\label{ref:replication}}
The source code with all associated instructions required for experimental replication (including data)  are made available via the following link: \modif{\url{https://github.com/submissionfse/DeepLSH}}.
